Persistent Homology with Improved Locality Information for more Effective Delineation

Persistent Homology (PH) has been successfully used to train networks to detect curvilinear structures and to improve the topological quality of their results. However, existing methods are very global and ignore the location of topological features. In this paper, we remedy this by introducing a new filtration function that fuses two earlier approaches: thresholding-based filtration, previously used to train deep networks to segment medical images, and filtration with height functions, typically used to compare 2D and 3D shapes. We experimentally demonstrate that deep networks trained using our PH-based loss function yield reconstructions of road networks and neuronal processes that reflect ground-truth connectivity better than networks trained with existing loss functions based on PH. Code is available at https://github.com/doruk-oner/PH-TopoLoss.

==> fig/mass.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure*}[b]
	\centering
	\begin{tabular}{@{} c c c @{}}
		\includegraphics[width=0.3\textwidth]{img/mas_im} &
		\includegraphics[width=0.3\textwidth]{img/mas_ce} &
		\includegraphics[width=0.3\textwidth]{img/mas_mse} \\
		{\it The input and the ground truth network} &
		\CE{} &
		\MSE{} \\
		
		\includegraphics[width=0.3\textwidth]{img/mas_dmt} & 
		\includegraphics[width=0.3\textwidth]{img/mas_malis} &
		\includegraphics[width=0.3\textwidth]{img/mas_bin}  \\
		\DMT{}& 
		\Malis{} &
		\HomoT{} \\
		
		\includegraphics[width=0.3\textwidth]{img/mas_dist} & 
		\includegraphics[width=0.3\textwidth]{img/mas_ours} &  \\
		\HomoR{}& 
		\Ours{} & \\
	\end{tabular}
\vspace{-3mm}
\caption{Qualitative results on the \MAS{} dataset.}
\label{fig:mass-comp}
\end{figure*}


==> fig/neurons.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure*}
	\centering
	\begin{tabular}{@{} c c c @{}}
		\includegraphics[width=0.3\textwidth]{img/neu_im} &
		\includegraphics[width=0.3\textwidth]{img/neu_ce} &
		\includegraphics[width=0.3\textwidth]{img/neu_mse} \\
		{\it The input and the ground truth network} &
		\CE{} &
		\MSE{} \\
		
		\includegraphics[width=0.3\textwidth]{img/neu_bin} & 
		\includegraphics[width=0.3\textwidth]{img/neu_dist} &
		\includegraphics[width=0.3\textwidth]{img/neu_ours}  \\
		\HomoT{}& 
		\HomoR{} &
		\Ours{}
	\end{tabular}
\vspace{-3mm}
\caption{Comparative results on the 3D \NEU{} dataset. }
\label{fig:neu-comp}
\end{figure*}


==> fig/ph_and_contribution.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

%\begin{figure}
%\center
%\includegraphics[width=\textwidth]{img/teaser_pers_diagrams}
%\caption{
%\label{fig:contribution}
%\MK{We need a figure like this: 1) that shows real prediction and ground truth 2) how individual homologies map to points in the persistence diagrams 3) matching of persistence diagrams 4) that the existing method clusters the points on the diagram together, and ours does not. 5) comparison of the segmentation results of a network trained with the existing loss and with ours. Do we need to show the loss function here? If so, how?}
%({\it Top}) 
%Persistent homology applied to comparison of the ground truth and the prediction of a road network.
%Individual homologies, in this case loops, give rise to points in the persistence diagram.
%Matching persistence diagrams takes the form of one-to-one matching between their points.
%The existing method clusters all the points in the ground truth diagram together, which provokes an erroneous match.
%In consequence, a loss function based on this matching (not shown in the figure) fails to penalize the road interruption and the false positive road.
%Our method distributes the points in the persistence diagram more evenly, preventing erroneous matches.
%As shown in the bottom of the figure, a loss function based on the proposed method improves the topology of the segmentation.
%}
%\end{figure}

\begin{figure}
	\centering
	\begin{tabular}{@{} c c c @{}}
		\includegraphics[width=0.281\textwidth]{img/teaser2_ims} &
		\includegraphics[width=0.323\textwidth]{img/teaser2_old} &
		\includegraphics[width=0.323\textwidth]{img/teaser2_our} 
		\\
		$(a)$ &
		$(b)$ &
		$(c)$ \\ 
          \\
		& \hspace{4mm}
		\includegraphics[width=0.288\textwidth]{img/teaser2_old_res} & \hspace{4mm}
		\includegraphics[width=0.288\textwidth]{img/teaser2_ours_res} 
		\\
        & \hspace{4mm}
		$(d)$ & \hspace{4mm}
		$(e)$ \\ 
	\end{tabular}
\caption{
	\label{fig:contribution}
	({\it a}) Persistent homology applied to comparison of the ground truth and the prediction of a road network.
	Individual homolog\ag{y classes}, in this case loops, give rise to points in the persistence diagram.
	Matching persistence diagrams takes the form of one-to-one matching between their points.
	({\it b}) The existing method clusters all the points in the ground truth diagram together, which provokes an erroneous match.
	In consequence, a loss function based on this matching (not shown in the figure) fails to penalize the road interruption and the false positive road.
	({\it c}) Our method distributes the points in the persistence diagram more evenly, preventing erroneous matches.
	({\it d})-({\it e}) Segmentations produced after the loss functions based on existing and proposed filtration methods, are applied, respectively.
	As shown in the bottom of the figure, a loss function based on the proposed method improves the topology of the segmentation.}
\end{figure}

==> fig/rt.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure*}[b]
	\centering
	\begin{tabular}{@{} c c c @{}}
		\includegraphics[width=0.3\textwidth]{img/rt_im} &
		\includegraphics[width=0.3\textwidth]{img/rt_mse} &
		\includegraphics[width=0.3\textwidth]{img/rt_seg} \\
		{\it The input and the ground truth network} &
		\MSE{} &
		\Segm{} \\
		
		\includegraphics[width=0.3\textwidth]{img/rt_rt} & 
		\includegraphics[width=0.3\textwidth]{img/rt_agata} &
		\includegraphics[width=0.3\textwidth]{img/rt_rcnn}  \\
		\RTracer{}& 
		\SegPath{} &
		\RCNN{} \\
		
		\includegraphics[width=0.3\textwidth]{img/rt_drm} &
		\includegraphics[width=0.3\textwidth]{img/rt_poly} &  
		\includegraphics[width=0.3\textwidth]{img/rt_malis}   \\
		\DRoad{}& 
		\PolyM{} &
		\Malis{} \\
	
		\includegraphics[width=0.3\textwidth]{img/rt_bin} &
		\includegraphics[width=0.3\textwidth]{img/rt_dist} &  
		\includegraphics[width=0.3\textwidth]{img/rt_ours}   \\
		\HomoT{}& 
		\HomoR{} &
		\Ours{} \\
	\end{tabular}
\vspace{-3mm}
\caption{Comparative results on the \RTD{} dataset.}
\label{fig:rtd-comp}
\end{figure*}


==> figmacro.tex <==
\newif\ifrgb
\rgbfalse

\newif\iffig
\figtrue

\newcommand{\figx}[2]
{
 \iffig
  \includegraphics[width=#1,keepaspectratio]{#2} 
 \else
   \parbox{#1}{#2} 
 \fi
}

\newcommand{\figy}[2]
{
 \iffig
  \includegraphics[height=#1,keepaspectratio]{#2}  
   \else
  \parbox{#1}{#2} 
 \fi
}

\newcommand{\figxy}[3]
{
 \iffig
  \includegraphics[width=#1,height=#2]{#3} 
 \else
   \parbox{#1}{#2}
  \fi
}

\newcommand{\figurecaption}[2]
{
\caption[]{\parbox[t]{#1}{#2}}
}

\newcommand{\fcaption}[1]
{
 \figurecaption{0.9\linewidth}{\small #1}
}

\newcommand{\figdir}[1]
{
\def\figurepath{#1}
}

\renewcommand{\topfraction}{1}
\renewcommand{\dbltopfraction}{1}
\renewcommand{\bottomfraction}{1}
\renewcommand{\textfraction}{.0}
\renewcommand{\floatpagefraction}{1}
\renewcommand{\dblfloatpagefraction}{1}


==> report.tex <==
\usepackage{named}

\usepackage{geometry}
\usepackage{times}
\usepackage{graphics}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{amsthm,amssymb}
\usepackage{color}

\geometry{
 a4paper,
 left=21mm,
 right=21mm,
 top=16mm,
 bottom=16mm,
 }
 
%\setlength{\oddsidemargin}{0.0in}
%\setlength{\topmargin}{-0.125in}
%\setlength{\textwidth}{6.25in}
%\setlength{\textheight}{8.75in}
%\parskip 6pt plus 3pt minus 2pt

\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\be}{\begin{enumerate}}
\newcommand{\ee}{\end{enumerate}}
\newcommand{\bd}{\begin{description}}
\newcommand{\ed}{\end{description}}
\newcommand{\im}{\item}
\newcommand{\comment}[1]{}
\newcommand{\missing}[1]{\begin{large} {\bf ADD:} {\em #1} \end{large}}
\newcommand{\note}[1]{\begin{center} \noindent\framebox{\begin{minipage}{8cm}{\bf #1}\end{minipage}}\end{center}\\}
\newcommand{\rmk}[1]{{\color{red}{ \bf #1}}}
\newcommand{\red}[1]{{\color{red}{#1}}}
\newcommand{\url}[1]{#1}

\newif\ifsubmit
\submitfalse

\newif\ifdraft
\draftfalse

\newcommand{\dspace}{\renewcommand{\baselinestretch}{1.5}\large\normalsize}
\newcommand{\sspace}{\renewcommand{\baselinestretch}{1.0}\large\normalsize}
\newcommand{\Section}[1]{\section{#1}}
\newcommand{\SubSection}[1]{\subsection{#1}}
\sspace

\renewcommand{\floatpagefraction}{1.0}


==> tab/results_abl_coeff.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table}[!h]
	\centering
	\caption{
		Impact of changing the learning coefficient of localized PH loss on the \MAS{} dataset.
		The window size is fixed to 64x64.
		\label{tab:results-abl-coeff}
	}
	\begin{tabular}{@{} p {0.14\columnwidth} @{}>{\centering\arraybackslash}p{1.0cm}>{\centering\arraybackslash}p{1.0cm}>{\centering\arraybackslash}p{1.0cm} >{\centering\arraybackslash}p{1.0cm}@{}>{\centering\arraybackslash}p{0.2cm}@{}>{\centering\arraybackslash}p{1.4cm} @{} }
		\cmidrule{2-7}
		
		& \multicolumn{4}{c}{Connectivity-oriented} && pixel-based \\
		
		\cmidrule{2-5}
		\cmidrule{7-7}
		
		$\alpha$ &    \APLS{} &       \TLTS &      \Junc &         \Betti &&        \CCQ \\
		\cmidrule{1-7}
		
		1e-3&
		64.9 &    46.0    &    77.1  &  1.21  &&    72.3 \\
		1e-2  & 
		\textbf{68.7} &    \textbf{50.6}    &    \textbf{79.2}  &  \textbf{0.90}  &&    \textbf{74.9} \\
		1e-1&
		67.1 &    48.9     &  77.8   &  0.94  &&    74.6 \\
		1e-0&
		 64.8     &  45.8   &    76.2        &  1.10  &&    72.0 \\
		\cmidrule{1-7}
		
	\end{tabular}
\end{table}



==> tab/results_abl_func.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table}[!h]
	\centering
	\caption{
		Performances of different height functions used for localized PH loss on the \MAS{} dataset.
		The learning coefficient is fixed to 1e-2 and window size to 64x64
		\label{tab:results-abl-function}
	}
	\begin{tabular}{@{} p {0.22\columnwidth} @{}>{\centering\arraybackslash}p{1.0cm}>{\centering\arraybackslash}p{1.0cm}>{\centering\arraybackslash}p{1.0cm} >{\centering\arraybackslash}p{1.0cm}@{}>{\centering\arraybackslash}p{0.2cm}@{}>{\centering\arraybackslash}p{1.4cm} @{} }
		\cmidrule{2-7}
		
		& \multicolumn{4}{c}{Connectivity-oriented} && pixel-based \\
		
		\cmidrule{2-5}
		\cmidrule{7-7}
		
		Height Function &    \APLS{} &       \TLTS &      \Junc &         \Betti &&        \CCQ \\
		\cmidrule{1-7}
		
		Dist.\ to a point &
		67.8  &    49.4    &   77.9  &  1.01  &&   73.6  \\
		Random Linear &
		\textbf{68.7} &    \textbf{50.6}    &    \textbf{79.2}  &  \textbf{0.90}  &&    \textbf{74.9} \\
		Fixed Linear &
		67.5 &    48.7    &    76.5  &  1.15  &&    73.0 \\
		Square &
		64.2 &    45.1    &    76.3  &  1.32  &&    70.3 \\
		
		\cmidrule{1-7}
		
	\end{tabular}
\end{table}



==> tab/results_abl_window.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table}[!h]
	\centering
	\caption{
		Impact of changing the window size when computing our localized loss on the \MAS{} dataset.
		The learning coefficient is fixed to 1e-2.
		\label{tab:results-abl-window}
	}
	\begin{tabular}{@{} p {0.14\columnwidth} @{}>{\centering\arraybackslash}p{1.0cm}>{\centering\arraybackslash}p{1.0cm}>{\centering\arraybackslash}p{1.0cm} >{\centering\arraybackslash}p{1.0cm}@{}>{\centering\arraybackslash}p{0.2cm}@{}>{\centering\arraybackslash}p{1.4cm} @{} }
		\cmidrule{2-7}
		
		& \multicolumn{4}{c}{Connectivity-oriented} && pixel-based \\
		
		\cmidrule{2-5}
		\cmidrule{7-7}
		
		Window Size &    \APLS{} &       \TLTS &      \Junc &         \Betti &&        \CCQ \\
		\cmidrule{1-7}
		
		8x8&
		62.1 &    41.9    &    73.0  &  2.84  &&    67.2 \\
		16x16  & 
		62.7 &    42.4    &    74.5  &  2.09  &&    68.8 \\
		32x32&
		65.4 &    45.7     &  77.1   &  1.17  &&    72.5 \\
		64x64&
		\textbf{68.7} &    \textbf{50.6}    &    \textbf{79.2}  &  \textbf{0.90}  &&    \textbf{74.9} \\
		\cmidrule{1-7}
		
	\end{tabular}
\end{table}


